SeeHow: Workflow Extraction from Programming Screencasts through Action-Aware Video Analytics

Programming screencasts (e.g., video tutorials on Youtube or live coding stream on Twitch) are important knowledge source for developers to learn programming knowledge, especially the workflow of completing a programming task. Nonetheless, the image nature of programming screencasts limits the accessibility of screencast content and the workflow embedded in it, resulting in a gap to access and interact with the content and workflow in programming screencasts. Existing non-intrusive methods are limited to extract either primitive human-computer interaction (HCI) actions or coarse-grained video fragments.In this work, we leverage Computer Vision (CV) techniques to build a programming screencast analysis tool which can automatically extract code-line editing steps (enter text, delete text, edit text and select text) from screencasts.Given a programming screencast, our approach outputs a sequence of coding steps and code snippets involved in each step, which we refer to as programming workflow. The proposed method is evaluated on 41 hours of tutorial videos and live coding screencasts with diverse programming environments.The results demonstrate our tool can extract code-line editing steps accurately and the extracted workflow steps can be intuitively understood by developers.

==> discussion.tex <==
\section{Discussion}
\subsection{Comparison with ActionNet and CodeTube}
\label{sec:comparisonwithactionnetcodetube}
\subsubsection{Methodology difference}
We use an illustrative example (see Fig.~\ref{fig:fragment}) to compare the key differences between our SeeHow method and two previous work (i.e. ActionNet~\cite{zhao2019actionnet} and CodeTube~\cite{ponzanelli2016too}), in terms of \textit{information granularity} and \textit{workflow extraction method}.

ActionNet detects actions between only two consecutive frames.
As shown in Fig.~\ref{fig:fragment}(a), this finest-grained analysis recognizes only a sequence of primitive HCI actions, such as mouse movement, character-level text changes, and window switching or popup.
Furthermore, ActionNet does not extract corresponding text content changed by the primitive actions.
Unless such primitive, content-agnostic actions are aggregated appropriately by an approach like our SeeHow, they do not intuitively correspond to any meaningful coding steps, and thus cannot directly support any developers' information needs, such as programming video search.

In contrast to the primitive HCI actions by ActionNet, CodeTube outputs coarse-grained video fragments based on the analysis of only frame content similarity.
As shown in Fig.~\ref{fig:fragment}(c), CodeTube detects only two long video fragments, one for editing configuration file, and the other for editing Splash activity class.
Because CodeTube is action-agnostic, a coarse-grained video fragment will involve many fine-grained coding steps, for examples, how to override the onCreate() method step by step.
The study by Bao et al.~\cite{bao2018vt} shows that such fine-grained coding steps are crucial for searching, exploring and learning programming video tutorials.

As shown in Fig.~\ref{fig:fragment}(b), our SeeHow method aims to extract coding steps at the line granularity in between the primitive HCI actions by ActionNet and the coarse-grained video fragments by CodeTube.
CodeMotion~\cite{khandwala2018codemotion} also attempts to recover code-line changes by comparing frame content changes.
However, because CodeMotion is action-agnostic, it suffers greatly from irrelevant frame content changes, such as window switching and popup.
Seehow uses the primitive actions detected by ActionNet to filter out such irrelevant frames.
Although instrumentation-based methods~\cite{bao2015activityspace,bao2018vt} can extract coding steps at the line granularity, they are limited by the underlying operating system's accessibility APIs.
In contrast, our SeeHow is a generic, vision-based method.

\subsubsection{Granularity difference}

\begin{table}
	\centering
	\caption{Performance of three methods}
	\begin{tabular}{cccc}
		\toprule
		\textbf{Method} & \textbf{ActionNet} & \textbf{SeeHow} & \textbf{CodeTube} \\
		\midrule
		Output Amount & 33727 & 5466 & 578 \\
		Mean fragment length & 2 & 7.62 $\pm$ 10.82 & 130.50 $\pm$ 114.43 \\
		\bottomrule
	\end{tabular}
	\label{tab:three} \\
	\scriptsize
\end{table}%

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{Fig/output.jpg}
	\caption{Search results of CodeTube (a) and SeeHow (b)}
	\label{fig:output}
\end{figure}

The most straightforward way to reflect the granularity difference is to analyze the outputs of the three methods.
We use ActionNet's source code and pretrained model from the author's Github repository \href{https://github.com/DehaiZhao/ActionNet_0}{\hlcolor{https://github.com/DehaiZhao/ActionNet\_0}} with default settings.
As CodeTube does not release source code, we implement it carefully with the top ranked parameters in the paper: $\alpha = 5\%$, $\beta = 15\%$ and $\gamma = 50s$, where $\alpha$ is minimum percentage of Longest Common Substring (LCS) overlap between two frames to consider them as containing the same code fragment, $\beta$ is minimum textual similarity between two fragments to merge them in a single fragment and $\gamma$ is minimum video fragment length.

We run the two methods on all 270 programming screencasts in our dataset and analyze the amount of output and the mean fragment length output by the three methods.
Table~\ref{tab:three} shows the results.
ActionNet has the highest amount of output (33,727) because it recognizes programming actions for adjacent two frames as long as there is a (small) change region between them, which is also the reason why its mean fragment length is two.
CodeTube finally extracts 578 video fragments from 270 screencasts, which is about 10 times less than the number of coding steps identified by SeeHow.
These video fragments have mean fragment length of 130.50 and standard deviation of 114.43 frames.
The high standard deviation is caused by the diversity of the tutorial authors' programming habits.
For example, some authors keep coding in one window even though the contents are not so coherent, while others switch window frequently in one video.
Our method output 5466 coding-step fragments with mean fragment length of 7.62 and standard deviation of 10.82 frames, which is between ActionNet and CodeTube.
The evaluation confirms that the identified coding step has high accuracy for code-line level changes and operations.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{Fig/dynamic.jpg}
	\caption{Example of dynamic programming behavior analysis}
	\label{fig:dynamic}
\end{figure}

\subsubsection{Search result difference}
\label{sec:searchresult}
Since CodeTube and SeeHow are designed for different purposes, their output results are significantly different.
CodeTube is a search engine for programming video tutorials that allows a user to retrieve video fragments extracted from long video tutorials.
Seehow is a workflow extractor and it outputs all coding steps that are manipulated by developer in programming screencasts.
We take Fig.~\ref{fig:output} as example, which shows key frames in the search results by CodeTube (Fig.~\ref{fig:output} (a)) and SeeHow (Fig.~\ref{fig:output} (b)) when input ``bitmap'' as search keyword.
We do not compare ActionNet in this section because it is designed for primary action recognition without text content extraction.
In Fig.~\ref{fig:output} (a), ``bitmap'' only appears on screen but is not the focus of the currently code editing.
What the developer actually do is to create a new method OnDraw() under MyBringBack().
As such, those video fragments contain little information about what the user expects for bitmap.
In Fig.~\ref{fig:output} (b), SeeHow returns a list of video fragments involving coding steps on bitmap-related content.
In these action-aware search results, the developer explains exactly how to call bitmap-related APIs and how to set parameters when using these APIs.
By watching these video fragments, users can accurately understand the details and the context of how to use a specific bitmap API.

\subsubsection{Summary}
SeeHow is essentially different from ActionNet and CodeTube in terms of the information granularity, and its output fills the gap between the primitive HCI actions by ActionNet and the coarse-grained video fragments by CodeTube.


\subsection{Scenarios to use SeeHow}
\label{sec:scenario}

SeeHow can extract line granularity coding steps from programming screencasts.
It could enable a wide range of applications in software engineering field and we envision two of these application scenarios in this paper.

\subsubsection{Video search}
Jenny is an Android development beginner who is still learning to develop some toy applications.
She is trying to use OnCreate() method to start an activity.
To do this, she not only reads Android development documents but also searches some online resources such as tutorial videos.
However, she finds it is hard for her to have a clear understanding on how to use the OnCreate() method because it is not well explained in these tutorial videos.
This issue is described in Section \ref{sec:searchresult}.
What Jenny needs indeed is the detailed explanations of a specific concept related to the API usage, which usually appear together with the manipulation of the API in the tutorials.
Unfortunately, searching video contents by keywords return too many fragments that contain OnCreate() but with no explanations.
Then she searches by keyword ``OnCreate'' on SeeHow and obtains a list of video fragments with clear indicators what the developer does on the code line with OnCreate().
These fragments illustrate how other developers create and edit OnCreate() method with proper explanations.
She inspects the text summary and picks the video fragments that she is interested in.
After watching these videos, Jenny gets deeper knowledge about how to use OnCreate() method in various conditions.
For example, when the author is typing ``OnCreate'', he also explains ``if you save the state of the application in a bundle, it can be passed back to onCreate if the activity needs to be recreated''.
SeeHow offers Jenny a fast and effective way to access a specific piece of API knowledge and makes learning process more smooth.

\subsubsection{Dynamic programming behavior analysis}

A time period later, Jenny has been familiar with Android development process and joins a project.
Fig.~\ref{fig:dynamic} shows key workflow steps in her development practice.
SeeHow can recognize a sequence of coding steps, including a class named LoginActivity is declared in Fig.~\ref{fig:dynamic} (a), an interface named MyApi is designed for posting email and password in Fig.~\ref{fig:dynamic} (b), user responses are added in Fig.~\ref{fig:dynamic} (c) and AuthViewModel class is created for displaying components such as login button in Fig.~\ref{fig:dynamic} (d).
By analyzing the four workflow steps above, SeeHow understands that Jenny has high probability to be developing a login page for an android application.
Then SeeHow recognizes that Jenny goes on progress bar in Fig.~\ref{fig:dynamic} (e), which is not the main functionality for login page. 
It finds an important step is required for completing the login function because most developers introduce this step (shown in Fig.~\ref{fig:dynamic} (f)) when developing such application.
Therefore, SeeHow displays a message to Jenny that a workflow step involving internet permission is recommended for current task and you can try to add the following code line <uses-permission android:name=``android.permission.INTERNET''>.
SeeHow acts as a intelligent programming assistant to help developers develop and debug, improving the work efficiency for developers.

Currently SeeHow does not include all the features that a intelligent programming assistant should have, but workflow extraction is the pre-requsite for such system.
It interprets what task the developer is doing by analyzing dynamic programming behavior and offers the most possible solutions to the issues.
We are actively working on such application scenarios based on the coding steps extracted by SeeHow.

\begin{comment}
\subsubsection{Summary}
SeeHow provides an effective way for video search and is helpful for downstream applications such as smart programming assistant.
However, it is not an improvement or replacement of CodeTube and ActionNet.
If users need to search videos that contain specific keywords, CodeTube can do it well.
When extracting low level programming actions, ActionNet should be considered.
If workflow information is required, SeeHow would be a good choice.
\end{comment}

\section{Threats to validity}
\textbf{Threats to internal validity} refer to factors internal to our studies that could have influenced our experimental results:

\begin{itemize}
	\item [(1)] 
	\emph{The evaluation of SeeHow:} The coding fragments and non-coding fragments are labeled manually for evaluating our method, which means error labels are inevitable.
	In order to minimize the human label errors, three annotators are recruited and label independently, and their labels achieve almost perfect agreement.
	The high agreement benefits from the explicit boundaries of coding steps at the line granularity.
	Some disagreements come from identifying whether the video fragments (e.g., typing a class name in configuration window) are relevant to coding.
	But the annotators were able to finally reach an agreement after discussion.
	
	\item [(2)]
	\emph{The knowledge background of annotators:} In RQ4, three developers were recruited to mark the correctness of the non-perfectly-aligned coding steps.
	A correct mark will be given if the developers believe they can understand the identified steps, even though these coding steps have inaccurate boundaries.
	%The three developers \zc{are not expert ??are expert?} in Java or Python, but a bias could potentially be introduced by the fact that they have several years' programming background.
	The three developers suggested that it is not difficult for them to understand the concepts in tutorial videos, especially those videos for beginners, by only watching a short fragment.
	A bias could be introduced because they have certain level of programming knowledge and experience.
	
\end{itemize}

\textbf{Threats to external validity} refer to the generalizability of the results in this study:

\begin{itemize}
	\item [(1)] 
	\emph{Scale of the dataset:} We construct the first dataset of the line-granularity coding steps, which covers two programming languages, 8 playlists, 270 videos and 41 hours duration.
	The dataset, far from covering all knowledge about programming, is a typical example of programming tutorial video, as those programming tutorials are not much different in their structure and content than others.
	In the future, we plan to collect more tutorial videos with different programming languages, tools and configurations to further evaluate SeeHow.
	In addition, labeling 41 hours video costs about one week for every annotator because of the required code-step granularity.
	For example, the annotator cannot exactly determine it is the end of a coding step when the author types the last character of a code line in frame $f_i$.
	Because more editing actions could be done in this code line.
	The annotator has to keep watching until the author starts editing a new line in frame $f_j$.
	Then he needs to revert back to $f_i$ and mark it as the end of a coding step.
	Such a large number of reverting operations makes the dataset very time consuming to create.
	\item [(2)]
	\emph{Noise in text recognition results:} We use computer vision and deep learning methods to recognize code from frames, which is inevitable to have error results.
	In \cite{bao2020psc2code}, the authors try to denoise code extracting results from programming screencasts by the statistical language model of a large corpus.
	However, we have to update the corpus when adding more programming screencasts and create a corpus for each programming language, which is an enormous work.
	We find that noises has no impact on our experimental results.
	Therefore, we ignore the denoise process and focus on the code recognition quality such as applying the deep learning based text detection \cite{zhou2017east} and text recognition \cite{shi2016end} methods in this work.
	The noisy results may affect the user experience of our SeeHow's web application when they read the extracted coding steps. 
	We plan to integrate the denoise process such as psc2code~\cite{bao2020psc2code} into our tool in the future.
	
	\item [(3)]
	\emph{Selection of OCR engine:} We apply EAST \cite{zhou2017east} and CRNN \cite{shi2016end} as OCR engines in this work. 
	There are many alternative methods such as google vision OCR \cite{google}, which has been shown to perform extremely well on programming screencasts and has been successfully used in previous work \cite{bao2020psc2code, moslehi2018feature, khormi2020study}.
	We also test google vision OCR and achieve similar performance with EAST and CRNN.
	EAST and CRNN run locally on GPU, and google vision OCR is cloud service.
	We finally choose EAST and CRNN mainly because of the following reasons:
	First, despite the network latency, the network security cannot be guaranteed, which is also a problem in software engineering field.
	Second, some devices with high security level are not allowed to connect to public network and it is infeasible to call google cloud service.
	Running source code locally is reliable and safe.
	Third, EAST and CRNN is free, but Google vision service is not.
	
\end{itemize}

